Compiler Discovered Dynamic Scheduling of Irregular Code in High-Level Synthesis

Dynamically scheduled high-level synthesis (HLS) achieves higher throughput than static HLS for codes with unpredictable memory accesses and control flow. However, excessive dataflow scheduling results in circuits that use more resources and have a slower critical path, even when only a part of the circuit exhibits dynamic behavior. Recent work has shown that marking parts of a dataflow circuit for static scheduling can save resources and improve performance (hybrid scheduling), but the dynamic part of the circuit still bottlenecks the critical path. We propose instead to selectively introduce dynamic scheduling into static HLS. This paper presents an algorithm for identifying code regions amenable to dynamic scheduling and shows a methodology for introducing dynamically scheduled basic blocks, loops, and memory operations into static HLS. Our algorithm is informed by modulo-scheduling and can be integrated into any modulo-scheduled HLS tool. On a set of ten benchmarks, we show that our approach achieves on average an up to 3.7$\times$ and 3$\times$ speedup against dynamic and hybrid scheduling, respectively, with an area overhead of 1.3$\times$ and frequency degradation of 0.74$\times$ when compared to static HLS.

==> Figures/BenchmarkTable.tex <==

\begin{table*}[!t]
% increase table row spacing, adjust to taste
% \renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{1.25pt}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
\caption{Evaluation of our approach against static scheduling (SS), dynamic scheduling \cite{josipovic_dynamatic_2022}, and DASS \cite{dass}. Three sets of benchmarks: 1--4 have control-dependent inter-iteration data dependencies, 5--8 have data-dependent memory accesses, and 9--10 have no data-dependent behavior. Area is shown as overhead over the respective SS baseline. NGM=Normalized Geometric Mean}
\label{table:benchmarkTable}
\centering
% Some packages, such as MDW tools, offer better commands for making tables
% than the plain LaTeX2e tabular which is used here.
\begin{tabular}{|c | >{\columncolor[gray]{0.9}}r>{\columncolor[gray]{0.9}}r>{\columncolor[gray]{0.9}}r | rrr | >{\columncolor[gray]{0.9}}r>{\columncolor[gray]{0.9}}r>{\columncolor[gray]{0.9}}r | rrrr | >{\columncolor[gray]{0.9}}r>{\columncolor[gray]{0.9}}r>{\columncolor[gray]{0.9}}r>{\columncolor[gray]{0.9}}r | rrrr|}
\hline
\multirow{2}{*}{} & \multicolumn{3}{>{\columncolor[gray]{0.9}}c|}{\textbf{LUTs $\times$SS}} & \multicolumn{3}{c|}{\textbf{REGs $\times$SS}} & \multicolumn{3}{>{\columncolor[gray]{0.9}}c|}{\textbf{DSPs $\times$SS}} & \multicolumn{4}{c|}{\textbf{FMax (MHz)}} & \multicolumn{4}{>{\columncolor[gray]{0.9}}c|}{\textbf{Cycles (thousands)}} & \multicolumn{4}{c|}{\textbf{Execution Time ($\mu$s)}} \\
% \cline{2-22}
\hhline{~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multicolumn{1}{>{\columncolor[gray]{0.9}}r}{\cite{josipovic_dynamatic_2022}} & \multicolumn{1}{>{\columncolor[gray]{0.9}}r}{\cite{dass}} & \multicolumn{1}{>{\columncolor[gray]{0.9}}r|}{Us}  
& \multicolumn{1}{r}{\cite{josipovic_dynamatic_2022}} & \multicolumn{1}{r}{\cite{dass}} & \multicolumn{1}{r|}{Us}  
& \multicolumn{1}{>{\columncolor[gray]{0.9}}r}{\cite{josipovic_dynamatic_2022}} & \multicolumn{1}{>{\columncolor[gray]{0.9}}r}{\cite{dass}} & \multicolumn{1}{>{\columncolor[gray]{0.9}}r|}{Us}
& \multicolumn{1}{r}{SS} & \multicolumn{1}{r}{\cite{josipovic_dynamatic_2022}} & \multicolumn{1}{r}{\cite{dass}} & \multicolumn{1}{r|}{Us}
& \multicolumn{1}{>{\columncolor[gray]{0.9}}r}{SS} & \multicolumn{1}{>{\columncolor[gray]{0.9}}r}{\cite{josipovic_dynamatic_2022}} & \multicolumn{1}{>{\columncolor[gray]{0.9}}r}{\cite{dass}} & \multicolumn{1}{>{\columncolor[gray]{0.9}}r|}{Us} 
& \multicolumn{1}{r}{SS} & \multicolumn{1}{r}{\cite{josipovic_dynamatic_2022}} & \multicolumn{1}{r}{\cite{dass}} & \multicolumn{1}{r|}{Us} \\

\hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  NO LSQ BELOW %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Intel SS LUTs=115, REG=205,
% Ours LUTs=136, REG=155,
% sparseMatrixPow 
1 & 2.3 & 1.4 & 1.2 & 2.6 & 1.1 & 0.8 & 2 & 1 & 1 & 415 & 111 & 111 & 334 & 1.8--11 & 0.3--11 & 0.3--11 & 0.1--11 & 4.3--26.5 & 2.7--99.1 & 2.7--99.1 & 0.3--32.9 \\

% SS: "alm"  : "168.7", "reg"  : "350",
% Ours 340, 500
% getTanhDouble 
2 & 1.1 & 1.1 & 1.7 & 1 & 1.3 & 1.4 & 1 & 1 & 1 & 371 & 111 & 111 & 372 & 38 & 1 & 1 & 1  & 102.4 & 9 & 9 & 2.7 \\

% SS: "alm"  : "723 "reg"  : "2110",
% Ours "alm"  : "1942.5 "reg"  : "4670",
% filterSum 
3 & 3.6 & 2 & 2.2 & 2.2 & 1.5 & 1.9 & 1 & 1 & 1 & 425 & 77 & 85 & 411 & 5 & 1--5 & 1--5 & 1--5  & 11.8 & 13--64.9 & 11.8--58.8 & 2.4--12.2 \\

% SS: "alm"  : "930.5 "reg"  : "2435",
% Our:  "alm"  : "2019 "reg"  : "5086",
% vecNormTrans 
4 & 3.1 & 2.8 & 2.1 & 2.2 & 2.1 & 2 & 4 & 1.4 & 1 & 374 & 90 & 106 & 379 & 12 & 6.1 & 6.7 & 6.1  & 32.1 & 67.8 & 63.2 & 16.1 \\

\hline
\textbf{NGM} & \textbf{2.3} & \textbf{1.7} & \textbf{1.7} & \textbf{1.9} & \textbf{1.5} & \textbf{1.4} & \textbf{1.7} & \textbf{1.1} & \textbf{1} & \textbf{1} & \textbf{0.24} & \textbf{0.25} & \textbf{0.94} & \textbf{1} & \textbf{0.14--0.34} & \textbf{0.14--0.34} & \textbf{0.09--0.34} & \textbf{1}  & \textbf{0.6--1.4} & \textbf{0.57--1.34} & \textbf{0.12--0.36} \\
\hline

% Intel SS LUTs=414, REG=548,
% Ours LUTs=750, REG=922,
% histogram 
5 & 2.4 & 2.4 & 1.1 & 1.9 & 2.4 & 1.4 & 1 & 1 & 1 & 356 & 60 & 68 & 168 & 9 & 1 & 1 & 1 & 25.3 & 16.7 & 14.7 & 6 \\

% SS: "alm"  : "192.0, "reg"  : "346",
% Our:  "alm"  : "376.8, "reg"  : "443",
% bubbleSort
6 & 8.6 & 9.1 & 2 & 5.9 & 6.2 & 1.3 & 1 & 1 & 1 & 447 & 64 & 59 & 168 & 20 & 10--20 & 10--20 & 10--20  & 44.7 & 156.2-312.5 & 169.5-339 & 59.5-119 \\

% SS: "alm"  : "169.6 "reg"  : "379",
% Our: 331, 625
% getTanh 
7 & 4.2 & 1.5 & 1.9 & 3 & 1.1 & 1.6 & 2 & 1 & 1 & 368 & 65 & 45 & 161 & 44-56 & 2.5--66 & 2.5--11 & 1--3.2  & 119.6--152.2 & 38.5--1015.4 & 55.6--244.4 & 6.2--19.9 \\

% SS: "alm"  : "358.1 "reg"  : "700",
% Ours: 567, 823
% BNN 
8 & 4.1 & 2.2 & 1.6 & 11.3 & 3.7 & 1.2 & 3 & 1 & 1 & 447 & 61 & 113 & 174 & 60 & 30 & 30 & 10  & 134.2 & 491.8 & 265.5 & 57.5 \\


\hline
\textbf{NGM} & \textbf{4.3} & \textbf{2.9} & \textbf{1.6} & \textbf{4.4} & \textbf{2.8} & \textbf{1.4} & \textbf{1.6} & \textbf{1} & \textbf{1}  & \textbf{1} & \textbf{0.16} & \textbf{0.17} & \textbf{0.42} & \textbf{1} & \textbf{0.2--0.5} & \textbf{0.2--0.32} & \textbf{0.12--0.18} & \textbf{1}  &  \textbf{1.28--3.26} &  \textbf{1.19--1.93} &  \textbf{0.29--0.43} \\
\hline

% covariance
9 & 3.4 & 1.6 & 1 & 3.4 & 1.6 & 1 & 1.8 & 1.8 & 1 & 434 & 86 & 100  & 434 & 68 & 72.9 & 84 & 68  & 156.7 & 847.7 & 840 & 156.7 \\
% gesummv 
10 & 1.6 & 1.3 & 1 & 1.6 & 1.3 & 1 & 2.2 & 1.7 & 1 & 410 & 113 & 163 & 410 & 65.8 & 262 & 68.8 & 65.8 & 160.5 & 2318.6 & 674.5 & 160.5 \\
\hline
\textbf{NGM} & \textbf{2.3} & \textbf{1.4} & \textbf{1} & \textbf{2.3} & \textbf{1.4} & \textbf{1} & \textbf{1.4} & \textbf{1.3} & \textbf{1} &  \textbf{1} & \textbf{0.23} & \textbf{0.3} & \textbf{1} & \textbf{1} & \textbf{2.07} & \textbf{1.13} & \textbf{1} & \textbf{1} & \textbf{8.84} & \textbf{4.75} & \textbf{1} \\
\hline


\end{tabular}
\end{table*}




==> Figures/BramDramIIsPlot.tex <==

\begin{figure}[h]
\centering
\subfloat[histogram in DRAM]{\includegraphics[width=0.24\textwidth]{Figures/ii_sim_hw_dram_exp_histogram.pdf}}%
\subfloat[histogram in BRAM]{\includegraphics[width=0.24\textwidth]{Figures/ii_sim_hw_bram_exp_histogram.pdf}}%

\caption{The impact of the LSQ Initiation Interval (II) on the number of simulation cycles (red) and on the execution time in hardware (green). On the left, the LSQ protects DRAM, on the right BRAM.}

\label{fig:bramDramII}
\end{figure}



==> Figures/ControlDependentStore.tex <==

\begin{figure}[!t]
    \centering
    \includegraphics[width=2.5in]{Figures/control_dependent_store.pdf}
    \caption{Test.}
    \label{fig_test}
\end{figure}

==> Figures/Deadlock.tex <==


\begin{figure}[t]
\centering

\includegraphics[width=0.45\textwidth]{Figures/deadlock.pdf}

\caption{The communication pattern after address generation decoupling.}

\label{fig:deadlock}
\end{figure}



==> Figures/DecoupledCFGFigure.tex <==


\begin{figure}[t]
\centering
% \vspace{-3em}
\subfloat[Fig. \ref{fig:MotivatingExampleCode} CFG.]{\includegraphics[width=0.117\textwidth]{Figures/OriginalCFG.pdf}\label{fig:OriginalCFG}}%
\hfill%
\subfloat[Decoupled CFG after our transformation.]{\includegraphics[width=0.36\textwidth]{Figures/DecoupledCFG.pdf}\label{fig:DecoupledCFG1}}%
% \hspace{0.4cm}
% \subfloat[]{\includegraphics[width=0.15\textwidth]{Figures/SwitchInSycl.pdf}\label{fig:PipeDiagramSwitchInSycl}}

% Switch implementation using SYCL pipes.
% Switch dataflow primitive
% SYCL pipes

\caption{A visual representation of dynamically scheduling one basic block from the code in fig. \ref{fig:MotivatingExample}..}

\label{fig:DecoupledCFG}
\end{figure}


==> Figures/DepPercentagePlot.tex <==


\begin{figure}[h]
\centering
\subfloat[histogram]{\includegraphics[width=0.25\textwidth, trim=0cm 0cm 1cm 0cm]{Figures/dep_percent_exp_histogram_hw.pdf}}%
\subfloat[sparseMatrixPower]{\includegraphics[width=0.25\textwidth, trim=0cm 0cm 1cm 0cm]{Figures/dep_percent_exp_spmv_hw.pdf}}


\caption{The relationship between the amount of real data hazards in a benchmark and its run time (lower is better). Our work is able to adapt to dynamic runtime conditions; the baseline static approach cannot.}

\label{fig:DepPercentagePlot}
\end{figure}



==> Figures/FullMuxTransform.tex <==


\begin{figure*}[t]
\centering

\subfloat[Original.]{\includegraphics[height=2cm]{Figures/FullMuxGetTanhA.pdf}}\label{fig:FullMuxGetTanhA}%
\hfill
\subfloat[Dynamically scheduled memory.]{\includegraphics[height=2cm]{Figures/FullMuxGetTanhB.pdf}\label{fig:FullMuxGetTanhB}}%
\hfill
\subfloat[Dynamically scheduled inner loop.]{\includegraphics[height=2cm]{Figures/FullMuxGetTanhC.pdf}\label{fig:FullMuxGetTanhC}}%
\hfill
\subfloat[Removing unnecessary pipe read stall.]{\includegraphics[height=2cm]{Figures/FullMuxGetTanhD.pdf}\label{fig:FullMuxGetTanhD}}%


\caption{An illustration of how a code (\textit{getTanh}) with a control-dependent inner loop and unpredictable memory accesses would be transformed by our approach.}

\label{fig:FullTransformation}
\end{figure*}


==> Figures/LSQDiagram.tex <==


\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Figures/lsq_diagram.pdf}

\caption{Interaction between the user kernel and our load-store queue.}

\label{fig:LSQDiagram}
\end{figure}



==> Figures/MuxTransform.tex <==


\begin{figure}[t]
\centering
% \vspace{-3em}
\includegraphics[width=0.49\textwidth]{Figures/mux_transform.pdf}

% \subfloat[]{\includegraphics[width=0.22\textwidth]{Figures/MuxBefore.pdf}}\label{fig:MuxBefore}%
% \hfill%
% \subfloat[]{\includegraphics[width=0.22\textwidth]{Figures/SwitchPrimitive.pdf}\label{fig:MuxAfter}}%
% \hspace{0.4cm}
% \subfloat[]{\includegraphics[width=0.15\textwidth]{Figures/SwitchInSycl.pdf}\label{fig:PipeDiagramSwitchInSycl}}

% Switch implementation using SYCL pipes.
% Switch dataflow primitive
% SYCL pipes

\caption{Mux insertion for control dependent data dependencies across decoupled CFGs.}

\label{fig:MuxTransformation}
\end{figure}


==> Figures/PipeDiagram.tex <==


\begin{figure}
\centering
% \vspace{-3em}
\subfloat[]{\includegraphics[width=0.13\textwidth]{Figures/pipe_diagram.pdf}\label{fig:PipeDiagramPipe}}%
\hfill%
\subfloat[]{\includegraphics[width=0.33\textwidth]{Figures/SwitchPrimitive.pdf}\label{fig:PipeDiagramSwitchPrimitive}}%
% \hspace{0.4cm}
% \subfloat[]{\includegraphics[width=0.15\textwidth]{Figures/SwitchInSycl.pdf}\label{fig:PipeDiagramSwitchInSycl}}

% Switch implementation using SYCL pipes.
% Switch dataflow primitive
% SYCL pipes

\caption{SYCL pipes implement a latency-insensitive communication protocol (a). They allow to build dynamic dataflow primitives, such as a switch (b).}

\label{fig:PipeDiagram}
\end{figure}


==> Figures/QsizesPlot.tex <==
% \subfloat[histogram]{%
% \begin{minipage}{0.5\textwidth}
% \centering
% \includegraphics[width=0.5\textwidth]{Figures/qsizes_exp_ALM_histogram.pdf}%
% \hfill
% \includegraphics[width=0.5\textwidth]{Figures/qsizes_exp_REG_histogram.pdf}
% \end{minipage}}%

% \subfloat[matrixPower]{%
% \begin{minipage}{0.5\textwidth}
% \centering
% \includegraphics[width=0.5\textwidth]{Figures/qsizes_exp_ALM_spmv.pdf}%
% \hfill
% \includegraphics[width=0.5\textwidth]{Figures/qsizes_exp_REG_spmv.pdf}
% \end{minipage}}%


\begin{figure}[h]
\centering
\subfloat[histogram]{\includegraphics[width=0.25\textwidth, trim=0cm 0cm 0.8cm 0cm]{Figures/qsizes_exp_ALM_histogram.pdf}}%
\subfloat[sparseMatrixPower]{\includegraphics[width=0.25\textwidth, trim=0cm 0cm 0.8cm 0cm]{Figures/qsizes_exp_ALM_spmv.pdf}}

\caption{The relationship between the number of resources used, the circuit frequency and the runtime of the benchmark as store queue sizes grow.}

\label{fig:qsizesPlot}
\end{figure}



==> Figures/StaticDynamaticAndThisApproach.tex <==

\begin{table}[t]
% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1.2}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
\caption{A comparison of our work against related work.}
\label{table:comparison_static_dynamic_ours}
\centering
% Some packages, such as MDW tools, offer better commands for making tables
% than the plain LaTeX2e tabular which is used here.
\begin{tabular}{l|r r r}
% hline
\textbf{Feature} &\textbf{Dynamatic \cite{josipovic_dynamatic_2022}} & \textbf{DASS \cite{dass}} & \textbf{This Work}\\
\hline
Scheduling & Fully dynamic HLS & Manual marking of static regions in dynamic HLS & Automatic extraction of dynamic regions in static HLS \\
% \hline
% \hline
\end{tabular}
\end{table}

% Memory Disam.            1, 0, 1       
% High Freq.               1, 1, 0       
% Low resource usage.      1(low overhead), 1, 0    

==> Figures/StoreQueue.tex <==


\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{Figures/store_queue.pdf}

\caption{The store queue Content-Addressable Memory (CAM) is a circular buffer carried though the pipeline in registers. The \texttt{isWaiting} flag indicates whether the \texttt{value} is safe to read. The \texttt{countdown} field indicates how many cycles need to pass before the store is committed to memory. The\texttt{ tail} points to the oldest entry which has not yet received a \texttt{value}; the \texttt{head} points to the next available entry where a new request can be enqueued.}

\label{fig:storeQueueStructure}
\end{figure}



==> Figures/ToolFlow.tex <==


\begin{figure}[t]
\centering
% \includegraphics[width=0.49\textwidth]{Figures/ToolFlowHorizontal.pdf}
\subfloat[]{\includegraphics[width=0.17\textwidth]{Figures/tool_flow.pdf}
\label{fig:ToolFlowTools}}
\hspace{0.2cm}
\subfloat[]{\includegraphics[width=0.23\textwidth]{Figures/ToolFlowCode.pdf}
\label{fig:ToolFlowCode}}

\caption{Our tool flow (a) for introducing dynamically scheduled memory operations; and pseudocode (b) of the how our approach would transform the motivating code from fig. \ref{fig:MotivatingExampleCode}.}
% \caption{Our tool flow for introducing dynamically scheduled memory operations.}

\label{fig:ToolFlow}
\end{figure}


